Identifying Coordinated Accounts on Social Media through Hidden Influence and Group Behaviours

Disinformation campaigns on social media, involving coordinated activities from malicious accounts towards manipulating public opinion, have become increasingly prevalent. Existing approaches to detect coordinated accounts either make very strict assumptions about coordinated behaviours, or require part of the malicious accounts in the coordinated group to be revealed in order to detect the rest. To address these drawbacks, we propose a generative model, AMDN-HAGE (Attentive Mixture Density Network with Hidden Account Group Estimation) which jointly models account activities and hidden group behaviours based on Temporal Point Processes (TPP) and Gaussian Mixture Model (GMM), to capture inherent characteristics of coordination which is, accounts that coordinate must strongly influence each other's activities, and collectively appear anomalous from normal accounts. To address the challenges of optimizing the proposed model, we provide a bilevel optimization algorithm with theoretical guarantee on convergence. We verified the effectiveness of the proposed method and training algorithm on real-world social network data collected from Twitter related to coordinated campaigns from Russia's Internet Research Agency targeting the 2016 U.S. Presidential Elections, and to identify coordinated campaigns related to the COVID-19 pandemic. Leveraging the learned model, we find that the average influence between coordinated account pairs is the highest.On COVID-19, we found coordinated group spreading anti-vaccination, anti-masks conspiracies that suggest the pandemic is a hoax and political scam.

==> alternate.tex <==




% Several studies have focused on the detection of individual malicious accounts, and bots i.e. automated accounts, from content and network features \cite{ferrara2016detection,sharma2019combating}. However, unlike bots, coordinated campaigns are different in that have been linked to human operators from information agencies; and previous works that analyzed the activities of such accounts, found that their features were not consistent over time, such as the language, content and web client usage \cite{luceri2020detecting,zannettou2019let}. Both these factors make it harder to define characteristic features to distinguish trolls from regular accounts. Recent works addressing the problem of troll detection propose to leverage deceptive linguistic cues \cite{ferrara2020types} or \cite{luceri2020detecting}.   



% Existing approaches, it is still an open challenge. the detection of coordinated accounts (troll farms) poses significantly different challenges. individual features, collective group behaviour (sync time assumption, coordination feature assumption). it is harder to define characteristic features or what constitutes coordination in trolls. Modeling account activities on social media. Can we automatically uncover coordinated campaigns from their activities? motivating example

% We propose AMDN, which does this. We detect and uncover characteristic patterns in influence structure and interactions/ the incentives. Evaluate on IRA (sota unsupervised from only activity patterns). Collect covid data. Analysis extensive on covid-19 disinformation campaigns (first work to do so).


  

% Such influence campaigns were found to be manipulating social media discussions by using tactics of defamation, persuasion, and polarization on one or more issues \cite{martin2019recent}. 

% behaviour of trolls varies over time: automatically unveiling their activity is not straightforward. 


% Are we also making an assumption on definition of coordination that our model picks up on? Group and activity traces instead of textual or metadata features (cite rose)

% * 3) motivation is to trigger large sharing of their ideologies to manipulate opinions (do they jointly promote so that the content gets more visibility and acceptance for re-sharing).

% * 4) do all of them share each others content or within that there are smaller cliques operating together? (do they also consistently share other people’s information). [may be they don’t engage with each other but just push things and engage with other users, trying to blend in]




%{\color{red} We apply AMDN-HAGE to model the coordinated campaign on real-world Twitter data about the 2016 U.S. Presidential Election (with complete annotation) and COVID-19 (without complete annotation). From our experiments, we get following important discoveries:
%\begin{itemize}
%    \item From the election data we find that although the interactions between coordinated users could last for a long time, they decrease significantly faster than the influence between normal users. This property makes coordinated accounts identifiable.
%    \item On COVID-19 dataset, we find presence of coordinated efforts spreading disinformation related to anti-vaccination, anti-masks, political conspiracies, and public health. %Meanwhile, some cues suggest that coordinated campaigns may also exist in the discussion of some normal topics.
%\end{itemize}
%}


==> method_copy.tex <==

\section{Method}

In this section, we introduce the proposed method for detecting coordinated accounts in disinformation campaigns on social media from collective group behaviours of the accounts.  

\textbf{Input.} The only input we consider are the activity traces of accounts on the social network available as a sequence of events ordered in time. The event sequences can be represented as $C_s = [(u_1, t_1), (u_2, t_2), (u_3, t_3), \cdots (u_n, t_n)]$ where the tuple $(u_i, t_i)$ corresponds to an activity by account $u_i$ at time $t_i$. The activities represent account actions on the network such as posting original content, re-sharing, or replying, commenting, and reacting to other posts. In this work, we assume that the type of action or features such as contents of the post or account metadata are not provided, although additional available features can be easily incorporated in the method. This basic information is the most easily available for any social network. Furthermore, we assume that there is no prior knowledge about the disinformation campaign and all the accounts coordinating to orchestrate the campaign are unknown and need to be detected given the activity traces of all accounts on the network. 

\subsection{Modeling account activities} 
In this section, we introduce the method AMDN (Attentive Mixture Density Network) to model account activities and interactions between accounts towards detecting coordinated campaigns. 

In contrast to individual behaviours, collective or group anomalous behaviours of malicious accounts involved in coordinated campaigns, can be useful towards detecting such campaigns, without access to partially uncovered accounts in the disinformation campaign. Although this approach to detecting coordinated campaigns has been exploited in previous works discussed earlier \cite{pacheco2020uncovering,cao2014uncovering,yu2015glad}, the main challenge lies in identifying what features constitute as suspicious coordinated behaviours. An example is, determining if a group of accounts collectively sharing similar hashtags over a period of time suggest malicious coordinated activities? This reliance on defined features introduces large number of false positives and prevents a principled solution to address the problem, with multiple heuristic design choices \cite{pacheco2020uncovering} to reduce false positives, and improve recall with assumed coordinated behaviours.

Here, we address these challenges by instead proposing to automatically discover coordinated behaviours from the activity traces of accounts on the network. To that end, we propose to model account activities or discrete network events in continuous time based on temporal point processes; and use the model to learn latent interactions between accounts, directly from the activities, to discover coordinated group anomalous behaviours. We discuss the details of the model and architecture in the following subsections.

\subsection{Preliminaries on temporal point processes}
A temporal point process (TPP) is a stochastic process
whose realization is a list of discrete events in continuous time $t \in \mathbb{R}^{+}$ \cite{daley2007introduction}. In the case of different event types (here, accounts), a marked temporal point process assigns a type or mark $u$ to each event \cite{du2016recurrent} and can be used to capture temporal dynamics of different event types. Temporal point processes are also equivalently represented as counting processes $N(t)$ indicating the number of event occurrences up to time $t$. The history of events in the sequence up to time $t$ are generally denoted as $H_t = \{(u_i, t_i) | t_i < t, u_i \in \mathcal{U} \}$ where $\mathcal{U}$ represents the set of event types. The conditional intensity function $\lambda(t|H_t)$ of a point process is defined as the instantaneous rate of an event in an infinitesimal window at time $t$, given the history i.e. $\lambda(t|H_t)dt= \mathbb{E}[dN(t)|H_t]$. The conditional density function of the $i^{\textrm{th}}$ event can be derived from the conditional intensity function \cite{du2016recurrent}, as,
\begin{equation}
    p(t|H_t) = \lambda(t|H_t) \exp \left( -\int_{t_{i-1}}^{t} \lambda (s|H_t) ds \right)
\end{equation}
In social network data, the widely used formulation of the conditional intensity function is the multivariate Hawkes Process (HP) \cite{zhou2013learning}, 
\begin{equation}
    \lambda_i(t|H_t) = \mu_i +  \sum_{t_j < t} \alpha_{i,j} \kappa(t - t_j)
\end{equation}
where $\lambda_i(t|H_t)$ is the conditional intensity of event type $i$ at time $t$ with base intensity $\mu_i > 0$ and mutually triggering intensity from past events where $\alpha_{i,j} > 0$ captures the influence of event type $j$ on $i$ and $\kappa$ is a decay kernel to model influence decay over time. $\mu$ and $\alpha$ are learnable parameters which can be inferred from the data by maximizing the likelihood (MLE) of observed event sequences.

\textbf{Neural point process models.} The Hawkes Process (HP) formulation \cite{zhou2013learning} assumes additive, positive influence from past events on future ones, generally with an exponential intensity function based on the exponential temporal decay kernel. It provides limited flexibility for capturing complex event sequences and triggering patterns between events. This has led to research efforts in neural network based point process models \cite{du2016recurrent}. The two forms of representing the point process models are either by modeling the conditional intensity function \cite{du2016recurrent,mei2017neural,zhangself,zuo2020transformer} or modeling directly the conditional density function \cite{shchur2019intensity,omi2019fully}. The added flexibility with neural network point process models comes with the cost of reduced interpretability of the interactions and influence between events and event types, compared to HP where inferred $\alpha_{ij}$ is an interpretable form of influence or triggering patterns between event types.

\subsection{Model architecture and training} 

\begin{figure}
    \centering
    \includegraphics[width=3.5in]{img/March.pdf}
    \caption{Architecture of proposed (AMDN) to model conditional density function of account activities on social media.}
    \label{fig:model_arch}
\end{figure}


\begin{table}[t]
    \centering
    \renewcommand*{\arraystretch}{0.8}
    \caption{Summary of neural point process models.}
    \label{tab:tpp}
    \begin{tabular}{l|p{1.2cm}|p{1cm}|p{1cm}|p{1cm}}
    \toprule
    Model & Flexible intensity function & 
    Closed-form likelihood &
    Long-range dependencies &  Inter-pretable Influence  \\
    \midrule
    HP \cite{zhou2013learning} & no & y & y & y \\
    RMTPP \cite{du2016recurrent} & limited & y & limited & no \\
    FullyNN \cite{omi2019fully} & y & y & limited & no \\
    LogNormMix \cite{shchur2019intensity} & y & y & limited & no \\
    SAHP \cite{zhangself} & limited & no & y & y \\
    THP \cite{zuo2020transformer} & y & no & y & y \\
    \midrule
    \textbf{AMDN} & y & y & y & y \\ 
    \bottomrule
    \end{tabular}
\end{table}

Existing neural network point process models suffer from different drawbacks (summarized in Table~\ref{tab:tpp}) with a trade-off between flexibility in modeling complex event sequences and functional forms of point process, expressivity in modeling long-range event dependencies, interpretability, and closed-form likelihood for estimating parameters with maximum likelihood estimation.

\textbf{Limitations of existing neural methods}  Methods SAHP and THP (Table ~\ref{tab:tpp} require Monte Carlo sampling to estimate an integral in the likelihood function used in MLE (discussed later), as their intensity formulation does not have closed form solutions;  which provides noisy gradients in training the model, reducing effectiveness. On the other hand, HP, RMTPP define specific functional forms, e.g. exponential for intensity parameterization to have closed form likelihoods but are limited in the flexibility of the selected functional form of the intensity. LogNormMix and FullyNN alleviate these issues by modeling the conditional density and cumulative density getting flexibility and closed-form likelihoods. However, the neural network parameterizations in RMTPP, LogNormMix, FullyNN are based on recurrent neural networks and cannot be directly used to examine the influence between events and event types, which is possible in the other methods. We address this by modeling the conditional density function with interpretable neural network parameterizations, so that the influence structure can be learned and examined to understand coordinated behaviours of malicious accounts. In addition, by choosing more expressive parameterizations, we improve the ability of the model to capture long range and more structured dependencies on historical events, improving event time and type predictions (discussed in the experiment results).

In the following paragraphs, we discuss and provide details of the model architecture of AMDN and training function for MLE.
\\\\
\textbf{Encoding event sequences with masked self-attention.} We model event sequences as temporal point processes with the stochastic random variable $\tau \in \mathbb{R}^+$ representing the inter-event time. We denote $p(\tau|H_\tau)$ as the probability density function of the random variable given the event history. In order to represent the history $H_\tau$, we can leverage representation learning with neural networks to automatically extract useful features when learning the parameters of the model, similar to neural point process approaches.

We encode the input sequence $S = \{(u_i, t_i)\}^{L}_{1}$ of $L$ events using a masked self-attention mechanism. As compared to recurrent neural networks (RNNs), self-attention based transformer models have been used extensively in natural language processing  \cite{vaswani2017attention}. 
\paragraph{Masked self-attention}
The weights of the self-attention mechanism can be computed with matrix operations as follows,
\begin{align}
\begin{split}
& A = \sigma (QK^T/\sqrt{d})
   \quad\mathrm{and}\quad 
H_{attn} = AV
\quad \\
& Q = X W_q, \hspace*{0.1cm} K = X W_k, \hspace*{0.1cm} V = X W_v
\end{split}
\end{align}
where $\sigma$ is the softmax activation to compute attention weights $A$ of each event pairwise with all other events in the input sequence $S$. $Q, K, V$ are the query, key, value matrices which are projections of the input representation $X \in \mathbb{R}^{L \times d}$ of the events in the sequence. $L$ is the sequence length, $d$ is the input feature dimension. Weights $W_q, W_k, W_v$ are learnable parameters. $\sqrt{d}$ is the scaling factor to prevent large attention weights due to dot-products in high-dimensional inputs. At the end, we apply layer normalization, dropout and feed-forward layer to $H_{attn}$ to get output $H_{out} \in \mathbb{R}^{L \times d}$.

The self-attention must capture the dependency of each event on the sequence of history events prior to it. Therefore, to prevent the model from looking into future events, we use masked self-attention by masking out the attention weights along the upper diagonal of $A$. The output representations of each event $i$ in the sequence is then a weighted linear combination of projections $V$ of the historical input events, prior to the event $i$ in the sequence.

\paragraph{Position, event and time encoding} The attention mechanism by itself does not retain ordering of the events in the input sequence. Therefore encoding \emph{positional information} in the input is necessary. We use the sine-cosine functions for each dimension $j$ of $m$-dimensional position encoding, proposed in \cite{vaswani2017attention}.
\begin{equation}
\begin{split}
    PE_{pos, 2j} = \sin (pos/10000^{2j/m}),
    &\quad\\
    \hspace*{0.1cm}
    PE_{pos, 2j+1} = \cos(pos/10000^{2i/m})
\end{split}
\end{equation}

We also need to represent the input \emph{event type} and time $(u_i, t_i)$ information. Since we do not include additional features of accounts, and rely only on the activity traces, we must represent the event type with its one-hot encoding, and get its embedding based on learnable embedding matrix $W_e \in \mathbb{R}^{|\mathcal{U}| x m}$ for all event types.

In addition, since events sequences consist of irregular events in time, which is different from sequences used in language models; it becomes necessary to additionally encode time intervals between events. We encode the \emph{temporal information} based on \cite{xu2019self} which allows translation-invariant temporal
kernel functions supported by functional analysis theorems. The kernel function
$\mathcal{K}:T \times T \rightarrow \mathbb{R}$ can be represented in terms of high-dimensional feature maps $\phi$ shown below, and decomposed into multiple periodic kernel functions of different frequencies $\omega$ to embed time information.
\begin{equation}
    \mathcal{K}(t_1, t_2) = \psi (t_1 - t_2) = \langle\ \phi(t_1), \phi(t_2)\rangle
\end{equation}
\begin{equation}
    \phi_{\omega}(t) = [\sqrt{c_1}, \cdots \sqrt{c_{2j}} \cos(j\pi t/\omega), \sqrt{c_{2j+1}} \sin(j\pi t/\omega) \cdots]
\end{equation}
\begin{equation}
    \phi(t) = [\phi_{\omega_1}(t), \phi_{\omega_2}(t) \cdots \phi_{\omega_k}(t)]^T
\end{equation}
In the translation-invariant kernel function, $c_i$ are chosen as free parameters, $\omega$ are set as frequencies at different intervals in a range, and $\phi_{\omega} \in \mathbb{R}^m$, with the time difference between events as input. Also, $\phi \in \mathbb{R}^m$ is obtained by summing along the frequency axis. We note that recent works SAHP and THP also similarly leveraged self-attention for encoding the event sequences, but proposing heuristic temporal encoding, as variants of positional encoding but for time.

The embedding $X_i$ of event $i$ from input $(u_i, t_i)$ with $e_{u_i}$ as one-hot encoding of event type $u_i$; is a concatenation of event, position and temporal embedding, as follows. $X$ is for the whole sequence, and is used as input to the masked self-attention mechanism.
\begin{equation}
    X_i = [e_{u_i} W_e, PE_{pos=i}, \phi(t_i - t_{i-1})]
\end{equation}

\paragraph{Event history context vector} The attention mechanism gives us representations of each event using attention over events prior to it. We can use the representation of the last event or a recurrent network layer over the attention outputs $H_{out} \in \mathbb{R}^{Lxd}$ to summarize events histories into context vectors $C \in \mathbb{R}^{Lxd}$ where $L$ is event sequence length. Each $c_i \in C$ is a context vector encoding history of events up to $t_i$ i.e. history $H_{t_i}$ of the temporal point process.
\\\\
\textbf{Conditional probability density function.} 
$p(\tau|H_\tau)$ mentioned earlier denotes the conditional probability density function of the random variable corresponding to the time $\tau \in \mathbb{R}^+$ of the next event given the history. The conditional density can be represented with any chosen functional form, and parameterized by the extracted context vector $c_i$ of event history up to event $i$. Since $\tau$ needs to be positive, \cite{shchur2019intensity} proposed to represent the conditional density with a mixture of log-normal distributions. A mixture distribution can allow learning of more flexible functional forms of the density function, not restricted to exponential or other monotonic functions. Therefore the PDF of inter-event time given history, based on \cite{shchur2019intensity},
\begin{equation}
p(\tau_i| w_i, \mu_i, s_i) = \sum_{k=1}^{K} w^k_i \frac{1}{\tau s^k_i \sqrt{2\pi}} \exp \left( -\frac{(\log \tau_i - \mu^k_i)^2}{2 (s^k_i)^2} \right)
\end{equation}
\begin{equation}
    w_i = \sigma(V_w c_i + b_w), \hspace*{0.2cm} s_i = \exp(V_s c_i + b_s), \hspace*{0.2cm} \mu_i = V_{\mu}  c_i + b_{\mu}
\end{equation}
where the mixture weights $w_i$, means $\mu_i$ and stddevs $s_i$ are parameterized by extracted context history $c_i$ and learnable $V, b$. $\sigma$ is softmax for mixture weights, and $\exp$ is positivity constraint. 

The parameters of the model including the parameters used to encode the history (denoted jointly as $\theta$) can be learned using \emph{maximum likelihood estimation} from observed event sequences, as the density can be differentiably evaluated at $t_i$ for events $i$ in the sequence and trained with gradient back-propagation.
\begin{equation}
    \theta^* = \textrm{argmax}_{\theta} \sum_{i=1}^{L} \left[ \log p_{\theta}(t_i|H_{t_i}) + \log p_{\theta}(u_i|H_{t_i}) \right]
\end{equation}

\subsection{Detecting coordinated accounts} The architecture of the AMDN model to model activities on social media is shown in Fig~\ref{fig:model_arch}. AMDN can model and predict the next event time and type on the network, and therefore learns to capture the mutual influence and interactions between accounts e.g. which account triggers or influences activities of another account. 

Therefore, the learned model can be used to identify \emph{collectively anomalous behaviours} of accounts based on their activity traces and inferred interactions; automatically discovered from the activity traces without any assumed coordination features. Coordinated accounts can exhibit different strategies for promoting content than regular accounts. Therefore, by clustering the learned event type (account) embeddings we can identify anomalous groups of accounts that are involved in coordinated campaigns to promote and amplify the spread of content with focused agenda of manipulating opinions through social media.

One advantage of encoding event histories based on masked self-attention in this context, is that it can extract structured and long-range dependencies in the event sequence more effectively than sequential RNNs. In social media activities, structured dependencies are especially prevalent, since single source posts might be shared by multiple accounts forming long chains of events that are strongly dependent on the source and not necessarily intermediate events. 

The other advantage is that it provides interpretable influence between events based on the attention weights across sequences. This is useful in this context for discovering and explaining behaviours of coordinated accounts in disinformation campaigns. We take the influence between event $i$ and $j$ to be $A_{ij}$ from the inferred attention weights. Then the influence between event types $u$ and $v$ are the average of the attention weights across all sequences in which $u$ is in the history of $v$. We examine these inferred influence structures in the experiments section.


% check reasons later (read attention is all you need paper, and ramausen paper, time kernel mapping how is it d-dimension after concat and dot product, why does clustering embeddings make sense for anomalous behaviours)

==> misc.tex <==
\begin{table*}[t]
    \centering
    \caption{Ablation Study Results of the Optimization Algorithm on detection of coordinated disinformation campaigns of Russian (IRA) interference in US Elections.}
    \label{tab:IRA_ab_opt}
    \renewcommand*{\arraystretch}{0.8}
    \begin{tabular}{l|l|c|c|c|c|c|c}
    \toprule
     Optimization & Method & AP & AUC & F1@TH0.5 & Prec@TH0.5 & Rec@TH0.5 & MaxF1  \\
    \midrule
    &AMDN-HAGE & $0.162\pm0.02$&$0.465\pm0.02$&$0.181\pm0.06$&$0.220\pm0.08$&$0.154\pm0.05$&$0.275\pm0.02$ \\
    Adam w/o pre-train&AMDN-HAGE + Kmeans &$0.299\pm0.03$&$0.796\pm0.02$&$0.212\pm0.05$&$0.252\pm0.07$&$0.183\pm0.04$&$0.495\pm0.02$ \\
    &AMDN-HAGE + NN (S) &
    $0.809\pm0.04$&$0.916\pm0.02$&$0.761\pm0.02$&$0.735\pm0.06$&$\pmb{0.795\pm0.03}$&$\pmb{0.805\pm0.01}$ \\
    \midrule
    &AMDN-HAGE & $0.799\pm0.04$&$0.895\pm0.03$&$0.726\pm0.04$&$0.861\pm0.05$&$0.630\pm0.05$&$0.757\pm0.03$\\
    Adam w/ pre-train&AMDN-HAGE + Kmeans &$0.783\pm0.07$&$0.933\pm0.02$&$0.742\pm0.04$&$0.847\pm0.06$&$0.663\pm0.05$&$0.776\pm0.03$ \\
    &AMDN-HAGE + NN (S) &
    $0.831\pm0.04$&$0.926\pm0.03$&$0.767\pm0.03$&$0.753\pm0.05$&$0.785\pm0.05$&$0.798\pm0.04$ \\
    \midrule
    &AMDN-HAGE & $0.804\pm0.03$&$0.898\pm0.02$&$0.699\pm0.05$&$\pmb{0.941\pm0.04}$&$0.558\pm0.06$&$0.758\pm0.04$ \\
    Proposed Algorithm&AMDN-HAGE + Kmeans & $0.818\pm0.04$&\pmb{$0.935\pm0.02$}&$0.731\pm0.04$&$0.913\pm0.03$&$0.611\pm0.05$&$0.776\pm0.03$\\
    &AMDN-HAGE + NN (S) &
    \pmb{$0.838\pm0.04$}&$0.926\pm0.03$&$\pmb{0.769\pm0.04}$&$0.752\pm0.05$&$0.789\pm0.05$&$0.799\pm0.04$\\
    \bottomrule 
    \end{tabular}
\end{table*}

%\begin{table*}[t]
%    \centering
%    \caption{Ablation Study Results of the Optimization Algorithm on detection of coordinated disinformation campaigns of Russian (IRA) interference in US Elections.}
%    \label{tab:IRA}
    % \renewcommand*{\arraystretch}{0.8}
%    \begin{tabular}{l|l|c|c|c|c|c|c|c}
%    \toprule
%      Method & Optimization & AP & AUC & F1 & Prec & Rec & MaxF1  \\
%    \midrule
%    &Adam w/o pre-train & $16.2\pm0.02$&$46.5\pm0.02$&$18.1\pm0.06$&$22.0\pm0.08$&$15.4\pm0.05$&$27.5\pm0.02$ \\
%    AMDN-HAGE&Adam w/ pre-train &$79.9\pm0.04$&$89.5\pm0.03$&$\pmb{72.6\pm0.04}$&$86.1\pm0.05$&$\pmb{63.0\pm0.05}$&$75.7\pm0.03$ \\
%    &Proposed Algorithm  &
%    $\pmb{80.4\pm0.03}$&$\pmb{89.8\pm0.02}$&$69.9\pm0.05$&$\pmb{94.1\pm0.04}$&$55.8\pm0.06$&$\pmb{75.8\pm0.04}$ \\
%    \midrule
%    &Adam w/o pre-train & $29.9\pm0.03$&$79.6\pm0.02$&$21.2\pm0.05$&$25.2\pm0.07$&$18.3\pm0.04$&$49.5\pm0.02$ \\
%    AMDN-HAGE + Kmeans&Adam w/ pre-train &$78.3\pm0.07$&$93.3\pm0.02$&$\pmb{74.2\pm0.04}$&$84.7\pm0.06$&$\pmb{66.3\pm0.05}$&$\pmb{77.6\pm0.03}$ \\
%    &Proposed Algorithm &
%    $\pmb{81.8\pm0.04}$&\pmb{$93.5\pm0.02$}&$73.1\pm0.04$&$\pmb{91.3\pm0.03}$&$61.1\pm0.05$&$\pmb{77.6\pm0.03}$ \\
%    \midrule
%    &Adam w/o pre-train & $80.9\pm0.04$&$91.6\pm0.02$&$76.1\pm0.02$&$73.5\pm0.06$&$\pmb{79.5\pm0.03}$&$\pmb{80.5\pm0.01}$ \\
%    AMDN-HAGE + NN (S)&Adam w/ pre-train &$83.1\pm0.04$&$\pmb{92.6\pm0.03}$&$76.7\pm0.03$&$\pmb{75.3\pm0.05}$&$78.5\pm0.05$&$79.8\pm0.04$ \\
%    &Proposed Algorithm  &
%    \pmb{$83.8\pm0.04$}&$\pmb{92.6\pm0.03}$&$\pmb{76.9\pm0.04}$&$75.2\pm0.05$&$78.9\pm0.05$&$79.9\pm0.04$ \\
%    \bottomrule 
%    \end{tabular}
%\end{table*}



% \begin{table*}[t]
%     \centering
%     \caption{Ablation Study Results of the Social Group Modeling on detection of coordinated disinformation campaigns of Russian (IRA) interference in US Elections.}
%     \label{tab:IRA_ab_joint}
%     \renewcommand*{\arraystretch}{0.7}
%     \begin{tabular}{p{1.2cm}|l|c|c|c|c|c|c}
%     \toprule
%       Joint Learning& Method & AP & AUC & F1@TH0.5 & Prec@TH0.5 & Rec@TH0.5 & MaxF1\\% & Macro@TH0.5 \\
%     \midrule
%     &AMDN + GMM(tied) & $0.787\pm0.05$&$0.894\pm0.03$&$0.631\pm0.06$&$\pmb{0.965\pm0.03}$&$0.472\pm0.07$&$0.738\pm0.05$\\%&$79.2\pm0.03$ \\
%     No&AMDN + Kmeans &$0.730\pm0.08$&$0.900\pm0.02$&$0.722\pm0.05$&$0.808\pm0.07$&$0.655\pm0.06$&$0.750\pm0.05$\\%&$83.9\pm0.03$ \\
%     &AMDN + NN (S) &
%     $0.810\pm0.04$&$0.915\pm0.02$&$0.726\pm0.04$&$0.705\pm0.06$&$0.753\pm0.05$&$0.761\pm0.04$\\%&$83.7\pm0.02$ \\
    
%     \midrule
%     &AMDN-HAGE & $0.804\pm0.03$&$0.898\pm0.02$&$0.699\pm0.05$&$0.941\pm0.04$&$0.558\pm0.06$&$0.758\pm0.04$\\%&$82.8\pm0.03$ \\
%     Yes&AMDN-HAGE + Kmeans &$0.818\pm0.04$&$\pmb{0.935\pm0.02}$&$0.731\pm0.04$&$0.913\pm0.03$&$0.611\pm0.05$&$0.776\pm0.03$\\%&$84.6\pm0.02$ \\
%     &AMDN-HAGE + NN (S) &
%     $\pmb{0.838\pm0.04}$&$0.926\pm0.03$&$\pmb{0.769\pm0.04}$&$0.752\pm0.05$&$\pmb{0.789\pm0.05}$&$\pmb{0.799\pm0.04}$\\%&$\pmb{86.2\pm0.02}$\\
%     \bottomrule 
%     \end{tabular}
% \end{table*}



% Since the back-end classifiers also influence the performance of coordinated account detection, in this paper, we discuss the detection performance of AMDN-HAGE with three different kinds of back-end classifier:
% \begin{enumerate}
%     \item AMDN-HAGE: We directly use the jointly learnt GMM model in HAGE part to output the group membership of each account. Then we predict the user belonging to the group with lower size and variance as coordinated account \item AMDN-HAGE + Kmeans: We train a Kmeans clsutering model on the learnt user embeddings and detect the coordinated users based on cluster membership exactly same as AMDN-HAGE.
%     \item AMDN-HAGE + NN (S): To evaluate the performance of AMDN-HAGE in supervised setting, we train a multi-layer perceptron to predict account label based on the learnt embedding of AMDN-HAGE.
% \end{enumerate}



%To verify the advantage of our novel optimization algorithm, we trained two variants with Adam. The first one is directly optimized by Adam optimizer with respect to the loss function $L(\theta_a,E,\theta_g)$ in Eq. \ref{eq:loss}. As for the second one, we first pre-train the model with line 1 to line 3 in Algorithm \ref{alg:training}, then jointly optimize the whole loss function with Adam. To make sure that we can acquire valid parameters, we constraint the covariance matrix $\Sigma$ to be a diagonal matrix and constraint each element greater than 1e-2 after each step. Above constraints are very crucial for the two variants. 




% \begin{algorithm}
%   \caption{Training Algorithm.}  
%   \label{alg:training}  
%   \begin{algorithmic}[1]
%   %\REQUIRE An neural network optimization algorithm $opt$.
%   % \ENSURE  The well-trained parameters $E,\theta_{a},\theta_{g}$.
    
%     \STATE Randomly initialize $\theta_a$ and $E$.
%     \STATE Acquire $\theta_{a}^{(0)}$ and $E^{(0)}$ by maximizing $\log P(C_s|U;E,\theta_{a})$.
%     \STATE Set $(\theta_a, E)$ as $(\theta_{a}^{(0)},E^{(0)})$.
%     \STATE Set $i$ as $1$ \COMMENT{Iteration index}.

%     \WHILE{not converged}
%     % \STATE Freeze $\theta_{a}$ and $E$.
%     \STATE Estimate $\theta_{g}^{(i)}$ by EM algorithm as $\textrm{argmax}_{\theta_{g}} \log p(U;E,\theta_{g})$.
%     \STATE Set $\theta_{g}$ as $\theta_{g}^{(i)}$ and freeze $\theta_{g}$.
%     \STATE Estimate $\theta_{a}^{(i)}$ and $E^{(i)}$ as $\textrm{argmax}_{\theta_a,E} \log p(C_s, U;\theta_g,\theta_a,E)$ by SGD/variant
%     % Acquire $\theta_{a}^(i)$ and $E^{(i)}$ by optimizing loss function $L(\theta_{a},E,\theta_{g}^{(i)})$ with a neural network optimization algorithm until convergence.
%     \STATE Set $(\theta_a, E)$ as $(\theta_{a}^{(i)},E^{(i)})$ and freeze $\theta_{a}$ and $E$.
%     \STATE $i \leftarrow i+1$.
%     \ENDWHILE
    
%   \end{algorithmic}  
% \end{algorithm} 
